Understanding Underrepresented Groups in Open Source Software

Context: Diversity can impact team communication, productivity, cohesiveness, and creativity. Analyzing the existing knowledge about diversity in open source software (OSS) projects can provide directions for future research and raise awareness about barriers and biases against underrepresented groups in OSS. Objective: This study aims to analyze the knowledge about minority groups in OSS projects. We investigated which groups were studied in the OSS literature, the study methods used, their implications, and their recommendations to promote the inclusion of minority groups in OSS projects. Method: To achieve this goal, we performed a systematic literature review study that analyzed 42 papers that directly study underrepresented groups in OSS projects. Results: Most papers focus on gender (62.3%), while others like age or ethnicity are rarely studied. The neurodiversity dimension, have not been studied in the context of OSS. Our results also reveal that diversity in OSS projects faces several barriers but brings significant benefits, such as promoting safe and welcoming environments. Conclusion: Most analyzed papers adopt a myopic perspective that sees gender as strictly binary. Dimensions of diversity that affect how individuals interact and function in an OSS project, such as age, tenure, and ethnicity, have received very little attention.

==> setup.tex <==
\usepackage{hyperref}
\hypersetup{pdfauthor={Name}} % to avoid warnings from hyperref

\usepackage{pdflscape}
\usepackage{longtable}
\usepackage{caption}
\usepackage{array}
\usepackage{relsize}
\usepackage{makecell}


\usepackage{tcolorbox}
\tcbuselibrary{skins}
\newenvironment{summarybox}
{\begin{tcolorbox}
[enhanced,arc=0mm,colback=gray!10,frame hidden,overlay unbroken={%
    \draw[thick,black] (interior.north west)--(interior.south west);
},left=2pt,right=0pt,top=0pt,bottom=0pt,before={\vspace{3pt}\noindent},after={\vspace{0pt}}]}
{\end{tcolorbox}}
\usepackage{xcolor}
\newenvironment{summary}
{\vspace{5pt}\noindent\begin{summarybox} Summary:}
{\end{summarybox}\vspace{-5pt}}

% \autoref
\renewcommand*{\sectionautorefname}{Section}%
\renewcommand*{\subsectionautorefname}{\sectionautorefname}%
\renewcommand*{\subsubsectionautorefname}{\subsectionautorefname}%
\renewcommand*{\paragraphautorefname}{\subsubsectionautorefname}%
\renewcommand*{\subparagraphautorefname}{\paragraphautorefname}%

\newcommand*{\tabindent}{ \hspace{3mm}}

\usepackage{xcolor}% http://ctan.org/pkg/xcolor

\usepackage{multirow}
\usepackage{todonotes}
% for dashed line in tables
\usepackage{tabu}% http://ctan.org/pkg/tabu

\usepackage{tabularx}% http://ctan.org/pkg/tabularx
\usepackage{booktabs}% http://ctan.org/pkg/booktabs
\makeatletter
\newcommand{\dashrule}[1][black]{%
  \color{#1}\rule[\dimexpr.5ex-.2pt]{4pt}{.4pt}\xleaders\hbox{\rule{4pt}{0pt}\rule[\dimexpr.5ex-.2pt]{4pt}{.4pt}}\hfill\kern0pt%
}
\newcommand{\rulecolor}[1]{%
  \def\CT@arc@{\color{#1}}%
}
\makeatother

\usepackage{makecell}

\usepackage{xspace}

\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%

\newcommand\numberToBeChecked[1]{\textcolor{black}{#1}}
\newcommand\textToBeChecked[1]{\textcolor{blue}{#1}}
\newcommand{\nbSeedPapers}{\numberToBeChecked{4}\xspace}
\newcommand{\nbManualSearch}{\numberToBeChecked{27}\xspace}
\newcommand{\nbPapersACM}{\numberToBeChecked{219}\xspace}
\newcommand{\nbPapersIEEE}{\numberToBeChecked{111}\xspace}
\newcommand{\nbPapersScopus}{\numberToBeChecked{379}\xspace}
\newcommand{\nbPapersFromAllEngines}{\numberToBeChecked{733}\xspace}
\newcommand{\nbPapersFromAllEnginesWithoutDuplicates}{\numberToBeChecked{631}\xspace}
\newcommand{\nbPapersAfterExclusionCriteria}{\numberToBeChecked{48}\xspace}
\newcommand{\nbPapersAfterInclusionCriteria}{\numberToBeChecked{42}\xspace}
\newcommand{\nbPapersFinalSelection}{\numberToBeChecked{42} \xspace}

\newcommand{\castor}[1]{\todo[inline,color=pink]{{\bf (castor note) }#1}}
\newcommand{\kiev}[1]{\todo[inline,color=blue!20!white]{{\bf (Kiev note) }#1}}
\newcommand{\reydne}[1]{\todo[inline,color=yellow!20!white]{{\bf (Reydne note) }#1}}
\newcommand{\rafa}[1]{\todo[inline,color=purple!20!white]{{\bf (Rafa note) }#1}}

\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

